Algorithms for Adversarially Robust Deep Learning

Given the widespread use of deep learning models in safety-critical applications, ensuring that the decisions of such models are robust against adversarial exploitation is of fundamental importance. In this thesis, we discuss recent progress toward designing algorithms that exhibit desirable robustness properties. First, we discuss the problem of adversarial examples in computer vision, for which we introduce new technical results, training paradigms, and certification algorithms. Next, we consider the problem of domain generalization, wherein the task is to train neural networks to generalize from a family of training distributions to unseen test distributions. We present new algorithms that achieve state-of-the-art generalization in medical imaging, molecular identification, and image classification. Finally, we study the setting of jailbreaking large language models (LLMs), wherein an adversarial user attempts to design prompts that elicit objectionable content from an LLM. We propose new attacks and defenses, which represent the frontier of progress toward designing robust language-based agents.

==> chapters/part-0-introduction/introduction.tex <==
% \part{Introduction}
% \epigraph{ ``This is a sample quote, illustrating the uncertainty principle in everyday life.''}{---Attribution}

\chapter*{Introduction}


==> chapters/part-1-perturbations/preliminaries.tex <==
\chapter{The problem of adversarial examples}



==> chapters/part-1-perturbations/semi-infinite/appendices/additional-experiments.tex <==
\section{Further experiments}\label{app:further-exps}

\subsection{MNIST}

We first consider the MNIST dataset~\cite{MNISTWebPage}.  All models use a four-layer CNN architecture trained using the Adadelta optimizer~\cite{zeiler2012adadelta}.  To evaluate the robust performance of trained models, we report the test accuracy with respect to two independent adversaries.  In particular, we use a 1-step and a 10-step PGD adversary to evaluate robust performance; we denote these adversaries by FGSM and PGD$^{10}$ respectively.  

A summary of the performance of DALE and various state-of-the-art baselines is shown in Table~\ref{tab:mnist-linf}.  Notice that DALE marginally outperforms each of the baselines in robust accuracy, while maintaining a clean accuracy that is similar to that of ERM.  This indicates that on MNIST, DALE is able to reach high robust accuracies without trading off in nominal performance.  This table also shows a runtime analysis of each of the methods.  Notably, DALE and TRADES have similar running times, which is likely due to the fact in our implementation of DALE, we use the same KL-divergence loss to search for challenging perturbations.

\begin{table}
\centering
\caption{\textbf{Accuracy and computational complexity on MNIST.}  In this table, we report the test accuracy and computational complexity of our method and various state-of-the-art baselines on MNIST.  In particular, all methods are trained using a four-layer CNN architecture, and we use a perturbation set of $\Delta = \{\bdelta\in\R^d : \norm{\bdelta}_\infty \leq 0.3\}$.  Our results are highlighted in gray.}\vspace{5pt}
\label{tab:mnist-linf}
\begin{tabular}{cccccccc}
\toprule
& & \multicolumn{3}{c}{Test accuracy (\%)} & \multicolumn{2}{c}{Performance (sec.)} \\ \cmidrule(lr){3-5} \cmidrule(lr){6-7}
\textbf{Algorithm} & $\bm\rho$ & \textbf{Clean} & \textbf{FGSM} & \textbf{PGD$^{10}$} & \textbf{Batch} & \textbf{Epoch} \\
\midrule
ERM & - & 99.3 & 14.3 & 1.46 & 0.007 & 3.47 \\ \midrule
FGSM & - & 98.3 & 98.1 & 13.0 & 0.011 & 5.48  \\
PGD & - & 98.1 & 95.5 & 93.1 & 0.039 & 18.2 \\
CLP & - & 98.0 & 95.4 & 92.2 & 0.047 & 21.9 \\
ALP & - & 98.1 & 95.5 & 92.5 & 0.048 & 22.0 \\
TRADES & - & 98.9 & 96.5 & 94.0 & 0.055 & 25.8 \\
MART & - & 98.9 & 96.1 & 93.5 & 0.043 & 20.4 \\
\midrule
\rowcolor{Gray} DALE & 1.0 & 99.1 & 97.7 & 94.5 & 0.053 & 25.4 \\
\bottomrule
\end{tabular} 
\end{table}


\subsection{CIFAR-10}

\begin{table}
    \centering
    \caption{\textbf{Accuracy and computational complexity on CIFAR-10.}  In this table, we report the test accuracy and computational complexity of our method and various state-of-the-art baselines on CIFAR-10.  In particular, all methods are trained using a ResNet-18 architecture, and we use a perturbation set of $\Delta = \{\bdelta\in\R^d : \norm{\bdelta}_\infty \leq 8/255\}$.  Our results are highlighted in gray.  Of note is the fact that our method advances the state-of-the-art both in adversarial and in clean accuracy.}\vspace{5pt}
    \label{tab:cifar-linf}
    \begin{tabular}{ccccccc} \toprule
        & & \multicolumn{3}{c}{Test accuracy (\%)} & \multicolumn{2}{c}{Performance (sec.)} \\ \cmidrule(lr){3-5} \cmidrule(lr){6-7}
         \textbf{Algorithm} & $\bm{\rho}$ & \textbf{Clean} & \textbf{FGSM} & \textbf{PGD$^{20}$} & \textbf{Batch} & \textbf{Epoch} \\ \midrule
         ERM & - & 94.0 & 0.01 & 0.01 & 0.073 & 28.1  \\ \midrule
         FGSM & - & 72.6 & 49.7 & 40.7 & 0.135 & 53.0 \\
         PGD & - & 83.8 & 53.7 & 48.1 & 0.735 & 287.9 \\
         CLP & - & 79.8 & 53.9 & 48.4 & 0.872 & 340.5 \\
         ALP & - & 75.9 & 55.0 & 48.8 & 0.873 & 341.2 \\
         TRADES & - & 80.7 & 55.2 & 49.6 & 1.081 & 422.0 \\
         MART & - & 78.9 & 55.6 & 49.8 & 0.805 & 314.1 \\ \midrule
         \rowcolor{Gray} DALE & 0.5 & \textbf{86.0} & 54.4 & 48.4 & 1.097 & 421.4 \\
         \rowcolor{Gray} DALE & 0.8 & 85.0 & 55.4 & 50.1 & 1.098 & 422.6 \\
         \rowcolor{Gray} DALE & 1.1 & 82.1 & 55.2 & \textbf{51.7} & 1.097 & 421.0 \\
         \bottomrule
    \end{tabular}
\end{table}

We next consider the CIFAR10 dataset~\cite{krizhevsky2009learning}.  Throughout this section, we use the ResNet-18 architecture trained using SGD, and we consider adversaries which can can generate perturbations $\bdelta$ lying within the perturbation set $\Delta = \{\bdelta\in\R^d : \norm{\bdelta}_\infty\leq 8/255\}$.  To this end, we use evaluate the robust performance of trained models using FGSM and PGD$^{20}$ adversaries.  For all of the classifiers trained using DALE, we use the KL-divergence loss for $\ell_\text{pert}$ and $\ell_\text{ro}$, and we use the cross-entropy loss for $\ell_\text{nom}$.

In Table~\ref{tab:cifar-linf}, we show a summary of our results on CIFAR-10.  One notable aspect of our results is that DALE trained with $\rho=0.8$ is the only model to achieve greater than 85\% clean accuracy and greater than 50\% robust accuracy.  This indicates that DALE is more successfully able to mitigate the trade-off between robustness and nominal performance.  And indeed, the baselines that have relatively high robust accuracy (TRADES and MART) suffer a significant drop in clean accuracy relative to DALE (-4.3\% for TRADES and -6.1\% for MART when compared with DALE trained with $\rho=0.8$).  Table~\ref{tab:cifar-linf} also shows a comparison of the computation time for each of the methods.  These results indicate that the computational complexity of DALE is on a par with TRADES.

\paragraph{A closer look at the trade-off between accuracy and robustness.}

We next study the trade-off between robustness and nominal performance of DALE for two separate architectures: ResNet-18 and ResNet-50.  In our formulation, the parameter $\rho$ explicitly captures this trade-off in the sense that a smaller $\rho$ will require a higher level of nominal performance, which in turn reduces the size of the feasible set.  This reduction has the effect of limiting the robust performance of the classifier.

In Table~\ref{tab:cifar-rho-trade-off}, we illustrate this trade-off by varying $\rho$ from 0.1 to 1.1.  For both architectures, the trade-off is clearly reflected in the fact that increasing the margin $\rho$ has the simultaneous effect of decreasing the clean accuracy and increasing the robust accuracy for both adversaries.  We highlight that for the ResNet-18 architecture, when the constraint is enforced with a relatively large margin (e.g., $\rho\geq 1.0$), DALE achieves nearly 52\% robust accuracy against \text{PGD}$^{20}$, which is nearly two percentage points higher than any of the baseline classifiers in Table~\ref{tab:mnist-and-cifar-linf}.  On the other hand, when the margin is relatively small (e.g., $\rho\leq 0.2)$, there is almost no trade-off in the clean accuracy relative to ERM in Table~\ref{tab:mnist-and-cifar-linf}, although as a result of this small margin, the robust performance takes a significant hit.  Interestingly, with regard to the classifiers trained using ResNet-50, it seems to be the case that the margin $\rho$ corresponding to the largest robust accuracy is different than the peak for ResNet-18.  

\begin{table}
    \centering
    \caption{\textbf{Evaluating the trade-off between robustness and accuracy.}  To evaluate the trade-off between robustness and nominal performance, we train ResNet-18 and ResNet-50 models on CIFAR-10 for different trade-off parameters $\rho$.  Notice that across both architectures, the impact of increasing $\rho$ is to simultaneously decrease clean performance and increase robust performance.}\vspace{5pt}
    \label{tab:cifar-rho-trade-off}
    \begin{tabular}{ccccccc} \toprule
         & \multicolumn{3}{c}{ResNet-18} & \multicolumn{3}{c}{Resnet-50}\\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
         $\bm\rho$ & \textbf{Clean} & \textbf{FGSM} & \textbf{PGD$^{\mathbf{20}}$} & \textbf{Clean} & \textbf{FGSM} & \textbf{PGD$^{\mathbf{20}}$} \\ \midrule
         0.1 & 93.0 & 35.6 & 1.50 & 93.8 & 23.9 & 16.7 \\
         0.2 & 92.4 & 43.6 & 11.9 & 93.7 & 20.5 & 16.3 \\
         0.3 & 88.7 & 42.4 & 31.2 & 90.1 & 43.0 & 24.8 \\
         0.4 & 86.4 & 50.9 & 44.3 & 86.2 & 50.5 & 38.4 \\
         0.5 & 86.0 & 54.4 & 48.4 & 86.5 & 50.1 & 42.6 \\
         0.6 & 85.6 & 54.6 & 49.0 & 86.1 & 57.7 & 52.0 \\
         0.7 & 85.3 & 56.2 & 50.3 & 84.7 & 57.0 & 51.4 \\
         0.8 & 83.8 & 55.4 & 50.1 & 84.3 & 56.4 & 50.8 \\
         0.9 & 83.8 & 56.0 & 51.3 & 83.9 & 55.9 & 51.2 \\ 
         1.0 & 82.2 & 54.7 & 51.2 & 82.1 & 54.2 & 50.1 \\ 
         1.1 & 82.1 & 55.2 & 51.7 & 80.4 & 52.3 & 49.9 \\ \bottomrule
    \end{tabular}
\end{table}


\paragraph{Impact of the number of Langevin iterations.}  In Table~\ref{tab:num-steps}, we study the impact of varying the number of Langevin iterations $L$.  For each row in this table, we train a ResNet-18 classifier with $\rho=1.0$; as before, we use the KL-divergence loss for $\ell_\text{pert}$ and $\ell_\text{ro}$, and we use the cross-entropy loss for $\ell_\text{nom}$.  As one would expect, when $L$ is small, the trained classifiers have relatively high clean accuracy and relatively low robust accuracy.  To this end, increasing $L$ has the simultaneous effect of decreasing clean accuracy and increasing robust accuracy. 

To offer a point of comparison, we also show the analogous results for PGD run using the cross-entropy loss, where $L$ is taken to be the number of steps of projected gradient ascent.  As each Langevin iteration of DALE effectively amounts to a step of projected gradient ascent with noise, we expect that the impact of varying $L$ in DALE will be analogous to the impact of varying the number of training-time PGD steps.  And indeed, as we increase $L$, the robust performance of PGD improves and the clean performance decreases.




\begin{table}
    \centering
    \caption{\textbf{Impact of the number of ascent steps.}  In this table, we show the impact of varying the number of Langevin steps used by DALE in lines~4-7 of Algorithm~\ref{L:algorithm}.  To offer a point of comparison, we also show the impact of varying the number of ascent steps for PGD.}\vspace{5pt}
    \label{tab:num-steps}
    \begin{tabular}{ccccccc} \toprule
         & \multicolumn{3}{c}{PGD$^{L}$} & \multicolumn{3}{c}{DALE} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
         $\mathbf{L}$ & \textbf{Clean} & \textbf{FGSM} & \textbf{PGD$^{\mathbf{20}}$} & \textbf{Clean} & \textbf{FGSM} & \textbf{PGD$^{\mathbf{20}}$}\\ \midrule
         1 & 92.9 & 52.3 & 23.7 & 87.2 & 46.6 & 39.0 \\
         2 & 90.9 & 49.9 & 36.6 & 85.4 & 53.6 & 47.1 \\
         3 & 87.7 & 50.6 & 41.5 & 84.0 & 55.0 & 50.2 \\
         4 & 84.5 & 52.2 & 43.3 & 82.8 & 55.0 & 50.7 \\
         5 & 83.6 & 53.5 & 47.9 & 82.5 & 54.9 & 50.7 \\
         10 & 83.8 & 53.7 & 48.1 & 82.2 & 54.7 & 51.2 \\
         15 & 82.9 & 54.0 & 48.0 & 81.0 & 54.7 & 51.0 \\
         20 & 83.0 & 54.4 & 48.3 & 81.0 & 54.7 & 51.4 \\ \bottomrule
        %  50 & & & & & & \\ 
    \end{tabular}
\end{table}



==> chapters/part-1-perturbations/semi-infinite/contents/theory.tex <==
\section{Dual robust learning}
\label{S:dual_robust_learning}

While empirically successful, in the previous section we argued that adversarial training is not without its shortcomings.  To this end, in this section, we develop the theoretical foundations needed to tackle the two challenges of~\eqref{P:robust}: 
%
\begin{enumerate}
    \item Finding worst-case perturbations, i.e., evaluating the robust loss defined in~\eqref{eq:rob-loss};
    \item Mitigating the trade-off between robustness and nominal performance.
\end{enumerate}
%
To address these challenges, we first propose a constrained optimization problem, which explicitly captures the trade-off between robustness and nominal performance.  In particular, we seek solutions to the following \emph{constrained} optimization problem:
%
\begin{mdframed}[roundcorner=5pt, backgroundcolor=yellow!8]
\begin{prob}[\textup{P-CON}]\label{P:main}
	P^\star \triangleq &\minimize_{\btheta \in \Theta} &&\E_{(\bv x, y) \sim \calD} \left[
	    	\max_{\dinD}\ \ell\big( f_{\btheta}(\xplusd), y \big)
	    \right]
    \\
	&\subjto &&\E_{(\bv x,y) \sim \calD} \left[ \ell\big(f_{\btheta}(\bv x), y\big) \right] \leq \rho
\end{prob}
\end{mdframed}
%
where~$\rho \geq 0$ is a desired nominal performance level.  At a high level, \eqref{P:main} seeks the most robust classifier $f_{\btheta}(\cdot)$ among those classifiers that have strong nominal performance.  In this way, \eqref{P:main} is directly designed to address the well-known trade-off between robustness and accuracy.  Thus,~\eqref{P:main} will be the central object of study in this paper.

At face value, the statistical constraint in~\eqref{P:main} is challenging to enforce in practice, especially given the well-known difficult in solving the unconstrained analog, e.g., \eqref{P:robust}, in practice.  To this end, our approach in this work is to use duality to obtain solutions for~\eqref{P:main} that generalize with respect to both adversarial and nominal performance~(see Section~\ref{S:csl}).  Before describing this approach, we emphasize that while we consider the nominal loss as a constraint, the theory and algorithms that follow also apply to constrained learning problems in which the objective and constraint of~\eqref{P:main} are swapped.

\subsection{Computing worst-case perturbations}
\label{S:sip}

Before tackling the constrained problem~\eqref{P:main}, we begin by consider its unconstrained version, namely, \eqref{P:robust}.  We start by writing~\eqref{P:robust} using an epigraph formulation of the maximum function to obtain the following semi-infinite program:
%
\begin{prob}\label{P:semi-infinite}
	P_\text{R}^\star = &\minimize_{\btheta \in \Theta,\, t \in L^p}
		&&\E_{(\bv x, y) \sim \calD} \!\big[ t(\bv x,y) \big]
	\\
	&\subjto &&\ell\big( f_{\btheta}(\xplusd), y \big) \leq t(\bv x,y)
		\text{,} \quad \text{for all } (\bv x, \pmb\delta, y) \in \calX \times \Delta \times \calY
		\text{.}
\end{prob}
%
Note that~\eqref{P:semi-infinite} is indeed equivalent to~\eqref{P:robust} given that
%
\begin{align}
    \max_{\dinD}\ell\big( f_{\btheta}(\xplusd), y \big) \leq t(\bv x,y) \iff \ell\big( f_{\btheta}(\xplusd), y \big) \leq t(\bv x,y) \:\: \text{for all } \dinD
        \text{.}
\end{align}
%
While at first it may seem that we have made~\eqref{P:main} more challenging to solve by transforming an unconstrained problem into an infinitely-constrained problem, notice that~\eqref{P:semi-infinite} is no longer a composite minimax problem.  Furthermore, it is \emph{linear} in~$t$, indicating that~\eqref{P:semi-infinite} should be amenable to approaches based on Lagrangian duality. Indeed, the following proposition shows that~\eqref{P:semi-infinite} can be used to obtain a statistical counterpart of~\eqref{P:robust}.

\begin{proposition}\label{T:robust_sip}
%
If~$(\bv x, y) \mapsto \ell\big( f_{\btheta}(\bv x), y \big) \in L^p$ for~$p\in(1,\infty)$, then~\eqref{P:robust} can be written as
%
\begin{prob}\label{P:primal_sip}
    P_\textup{R}^\star = \min_{\btheta \in \Theta}\ p(\btheta)
    	\text{,}
\end{prob}
%
for the primal function
%
\begin{equation} \label{E:primal_function}
	p(\btheta) \triangleq \max_{\lambda \in \calP^q}\ %
    \E_{(\bv x, y)\sim\calD} \left[
    	\E_{\bdelta \sim \lambda(\bdelta | \bv x, y)} \left[ \ell(f_{\btheta}(\bv x + \bdelta), y) \right]
    \right]
    	\text{,}
\end{equation}
%
where $q$ satisfies~$(1/p) + (1/q) = 1$ and~$\calP^q$ is the subspace of~$L^q$ containing functions $\lambda(\bdelta|\bv x,y)$ satisfying the following properties for almost every~$(\bv x, y) \in \Omega$:
%
\begin{enumerate}
    \item[(1)] $\lambda(\bdelta|\bv x,y)$ is non-negative almost everywhere;
    \item[(2)] $\lambda(\bdelta|\bv x,y)$ is absolutely continuous with respect to $\fkp$, i.e., $\fkp(\bv x, y) = 0 \Rightarrow \lambda(\bdelta | \bv x, y) = 0$;
    \item[(3)] $\lambda(\bdelta|\bv x,y)$ integrates to one, i.e., $\int_\Delta \lambda(\bdelta | \bv x, y) d\bdelta = 1$.
\end{enumerate}
%


\end{proposition}

\begin{proof}
    The proof is provided in Appendix~\ref{app:proof-prop-3.1}.
\end{proof}

\noindent Informally, Proposition~\ref{T:robust_sip} shows that the standard robust learning problem in~\eqref{P:robust} can be recast as a problem of optimizing over a set of probability distributions $\calP^q$ taking support over the perturbation set $\Delta$.  This establishes an equivalence between the traditional robust learning problem~\eqref{P:robust}, where the maximum is taken over perturbations $\bdelta\in\Delta$ of the input, and its stochastic version~\eqref{P:primal_sip}, where the maximum is taken over a conditional distribution of perturbations $\bdelta\sim\lambda(\bdelta|\bv x,y)$, where the only additional constraint is that $\lambda$ should be absolutely continuous with respect to the data density $\fkp$.

As we remarked in Section~\ref{S:problem}, for many modern function classes, the task of evaluating the adversarial loss $\ell_\text{adv}$ is a nonconcave optimization problem, which is challenging to solve in general.  Thus, Proposition~\eqref{T:robust_sip} can be seen as lifting the nonconcave inner problem $\max_{\delta\in\Delta} \ell(f_{\btheta}(\bv x),y)$ to the equivalent \emph{linear} optimization problem in~\eqref{E:primal_function} over probability distributions $\lambda\in\calP^q$.  This dichotomy parallels the one that arises in PAC vs.\ agnostic PAC learning. Indeed, while the former seeks a deterministic map~$(\btheta, \bv x, y) \mapsto \bdelta$, the latter considers instead a distribution of perturbations over~$\bdelta | \bv x, y$ parametrized by~$\btheta$. In fact, since~\eqref{P:primal_sip} is obtained from~\eqref{P:robust} through semi-infinite duality\footnote{For details, see the proof of Proposition~\ref{T:robust_sip} in Appendix~\ref{app:proof-prop-3.1}.}, the density of this distribution is exactly characterized by the dual variables~$\lambda$.

It is also worth noting that while~\eqref{P:primal_sip} was obtained using Lagrangian duality, it can also be seen as a \emph{linear lifting} of the maximization in~\eqref{eq:rob-loss}. From this perspective, while recovering~\eqref{eq:rob-loss} would require~$\lambda$ to be atomic, Proposition~\ref{T:robust_sip} shows that this is in fact not necessary as long as~$\ell(f_{\btheta}(\bv x), y)$ is an element of~$L^p$.  That is, because $\calP^q$ does not contain any Dirac distributions, the optimal distribution $\lambda^\star$ for the maximization problem in~\eqref{E:primal_function} is \emph{non-atomic}. Furthermore, observe that Proposition~\ref{T:robust_sip} does not account for~$p \in \{1,\infty\}$ for conciseness only, since their dual spaces are not isomorphic to~$L^q$ for any~$q$. Nevertheless, neither of the dual spaces~${L^1}^*$ or ${L^\infty}^*$ contain Dirac distributions, meaning that $\lambda^\star$ would remain non-atomic.

A final point of interest regarding Proposition~\ref{T:robust_sip} is that a variety of training formulations can be seen as special cases of this composite optimization problem.  In particular, for particular suboptimal choices of this distribution, paradigms such as random data augmentation and distributionally robust optimization can be recovered.  To streamline our presentation, we defer these connections to Appendix~\ref{app:connections}.



\subsection{Exact solutions for the outer maximization in Problem \texorpdfstring{\eqref{P:primal_sip}}{(PII)}}  While~\eqref{P:primal_sip} provides a new, infinitely-constrained alternative formulation for~\eqref{P:robust}, the fact  remains that the objectives of both~\eqref{P:primal_sip} and~\eqref{P:robust} involve the solution of a non-trivial inner maximization. However, whereas the maximization problem in~\eqref{P:robust} is a finite-dimensional optimization problem which is nonconcave for most modern function classes, the maximization in~\eqref{P:primal_sip} is a linear, variational problem regardless of the function class. We can therefore leverage variational duality theory to obtain a full characterization of the optimal distribution~$\lambda^\star$ when~$p = 2$.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{imgs/opt-pert.png}
        \caption{\textbf{Inner maximization in~\eqref{P:robust}.}  In~\eqref{P:robust}, for each $(x,y)\sim\mathcal{D}$ we seek a perturbation $\delta^\star\in\Delta$ which causes the classifier $f_{\btheta}$ to have high loss.  This can be interpreted as placing a Dirac measure $\lambda$ at $\delta^\star$ in~\eqref{P:primal_sip}, as shown above.}
        \label{fig:opt-pert}
    \end{subfigure}\quad
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=0.8\textwidth]{imgs/opt-dist.png}
        \caption{\textbf{Inner maximization in~\eqref{P:primal_sip}.}  In~\eqref{P:primal_sip}, for each $(x,y)\sim\mathcal{D}$ we seek a distribution $\lambda^\star$ over perturbations $\delta\in\Delta$.  Notably, the set $\calP^2$ does not contain any Dirac distributions, meaning that we can recover~\eqref{eq:rob-loss} with a non-atomic $\lambda^\star$.}
        \label{fig:opt-dist}
    \end{subfigure}
    \caption{\textbf{Comparing the inner maximizations of \eqref{P:robust} and \eqref{P:primal_sip} for $p=q=2$.}  In both plots, we illustrate the optimal perturbation distributions for~\eqref{P:robust} and~\eqref{P:primal_sip} in the special case of $p=q=2$.  One key aspect of our results is that the optimal distribution $\lambda^\star$ in~\eqref{P:primal_sip} is a non-atomic distribution.}
    \label{fig:compare-probs}
\end{figure}

\begin{proposition}[Optimal distribution for~\eqref{P:primal_sip}]\label{T:lambda_star}
%
Let~$p = 2$~(and~$q = 2$) in Proposition~\ref{T:robust_sip}, and let $[z]_+ = \max(0,z)$. For each~$(\bv x,y) \in \calX \times \calY$, there exists constants~$\gamma(\bv x,y) > 0$ and~$\mu(\bv x,y) \in \setR$ such that
%
\begin{equation}\label{E:lambda_star}
	\lambda^\star(\bdelta | \bv x, y) = \left[ \frac{\ell(f_{\btheta}(\bv x + \bdelta), y) - \mu(\bv x,y)}{\gamma(\bv x,y)} \right]_+
		\text{,}
\end{equation}
%
is a solution of the maximization in~\eqref{E:primal_function}. In particular, the value of~$\mu(\bv x,y)$ is such that
%
\begin{equation} \label{eq:mu-and-gamma}
	\int_\Delta \left[ \ell(f_{\btheta}(\bv x + \pmb \delta), y) - \mu(\bv x,y) \right]_+ d\bdelta = \gamma(\bv x,y)
		\text{, for all } (\bv x,y) \in \calX \times \calY
		\text{.}
\end{equation}
%
\end{proposition}

\begin{proof}
	The proof is provided in Appendix~C.
\end{proof}

\noindent Hence, in the particular case of~$(\bv x, y) \mapsto \ell\big( f_{\btheta}(\bv x), y \big)\in L^2$, we can obtain a closed-form expression for the distribution $\lambda^\star$ that maximizes the objective of~\eqref{P:primal_sip}.  Moreover, this distribution turns out to be proportional to a truncated version of the loss of the classifier.   Note that the assumption that the loss belongs to $L^2$ is mild given that the compactness of~$\calX$, $\calY$, and~$\Delta$ imply that~$L^{p_1} \subset L^{p_2}$ for~$p_1 > p_2$. It is, however, fundamental to obtain the closed-form solution in Proposition~\ref{T:lambda_star} since it allows~\eqref{E:primal_function} to be formulated as a strongly convex constrained problem whose primal solution~\eqref{E:lambda_star} can be recovered from its dual variables~(namely, $\gamma$ and~$\mu$).

To illustrate this result, it's useful to consider two particular \emph{suboptimal} choices for the constants $\mu$ and $\gamma$ described in Proposition~\ref{T:lambda_star}.  \vspace{5pt}

\noindent\textbf{Special case I: Over-smoothed $\lambda^\star$.}  To begin, we consider the case when $\gamma(\bv x,y)$ is taken to be a normalizing constant $\int_\Delta \ell(f_{\btheta}(\bv x+\bdelta),y) d\bdelta$ be for each $(\bv x,y)\in\Omega$.  As the loss function $\ell$ is non-negative by assumption, equation~\eqref{eq:mu-and-gamma} implies that $\mu(\bv x,y) = 0$ for each $(\bv x,y)\in\Omega$.  Therefore, the distribution defined in~\eqref{E:lambda_star} can be written as 
%
\begin{align}
    \lambda(\bdelta|\bv x,y) = \frac{\ell(f_{\btheta}(\bv x + \bdelta), y)}{\int_\Delta \ell(f_{\btheta}(\bv x + \bdelta), y)d\bdelta}, \label{eq:sampling-lambda}
\end{align}
%
meaning that $\lambda(\bdelta|\bv x,y)$ is exactly proportional to the loss $\ell(f_{\btheta}(\bv x+\bdelta),y)$ on a perturbed copy of the data.  Thus, for this choice of $\gamma$ and $\mu$, the distribution $\lambda$ in~\eqref{eq:sampling-lambda} is an over-smoothed version of the optimal distribution $\lambda^\star$.  In our experiments, we will use this over-smoothed approximation of $\lambda^\star$ to derive an MCMC-style sampler, which yields state-of-the-art performance on standard benchmarks.\vspace{5pt}

\noindent\textbf{Special case II: Under-smoothed $\lambda^\star$.}  It is also of interest to consider the case in which $\gamma$ approaches zero.  In the proof of Proposition~\ref{T:lambda_star}, we show that the value of $\mu$ is fully determined by $\gamma$, and that $\gamma$ is directly related to the smoothness of the optimal distribution; in fact, $\gamma$ is equivalent to a bound on the $L^2$ norm of $\lambda^\star$.  In this way, as we take $\gamma$ to zero, we find that $\mu$  approaches $\ell(f_{\btheta}(\mathbf x+\bm\delta),y)$, meaning that the distribution is truncated so that mass is only placed on those perturbations $\bdelta$ which induce the high loss.  Thus, in the limit, $\lambda$ approaches a highly under-smoothed atomic distribution concentrated entirely at a perturbation $\delta^\star$ that maximizes the loss, i.e.,
%
\begin{align}
    \lambda(\bm\delta|\mathbf x,y) = \begin{cases} 
        1 &\quad \bdelta^\star \in\argmax_{\bdelta\in\Delta} \ell(f_{\btheta}(\bv x + \bdelta), y) \\
        0 &\quad\text{otherwise.}
    \end{cases}
\end{align}
%
Interestingly, this is the same distribution that would be needed to recover the solution to the inner maximization as in~\eqref{P:main}.  This connection, which we illustrate in Figure~\ref{fig:compare-probs}, highlights the fact that although recovering the optimal perturbation $\delta^\star$ in~\eqref{P:main} would require $\lambda^\star$ to be atomic, the condition that $\gamma > 0$ means that $\lambda^\star$ will be non-atomic.\vspace{5pt}

These two special cases illustrate the fundamental difference between~\eqref{P:robust} and~\eqref{P:primal_sip}: Whereas in~\eqref{P:robust} our goal is to search for worst-case perturbations, in~\eqref{P:primal_sip} we seek a method that will allow us to sample perturbations $\bm\delta$ from the non-atomic perturbation distribution $\lambda^\star$.  Thus, given a method for sampling $\delta\sim\lambda^\star(\bm\delta|\mathbf x,y)$, the max in~\eqref{P:robust} can effectively be replaced by an expectation, allowing us to consider the following optimization problem:
%
\begin{prob}\label{P:replace-max}
    P_\textup{R}^\star = \min_{\btheta \in \Theta} \E_{(\bv x,y)\sim\calD} \left[ \E_{\bdelta\sim\lambda^\star(\bdelta|\bv x, y)} \left[ \ell(f_{\bm\theta}(\bv x+\bdelta,y) \right] \right].
\end{prob}
%
Notice that crucially this problem is non-composite, in the sense that it no longer contains an inner maximization.  To this end, in Section~\ref{S:algorithm}, we propose a scheme that can be used to sample from $\lambda^\star$ toward evaluating the inner expectation in~\eqref{P:replace-max}.




\section{Solving the constrained learning problem}
\label{S:csl}

So far, we have argued that~\eqref{P:main} captures the problem of finding the most robust model with high nominal performance, and we have shown the the minimax objective of~\eqref{P:main} can be rewritten as a stochastic optimization problem over perturbation distributions.  In this section, we address the distinct yet related issue of satisfying the constraint in~\eqref{P:main}, which is a challenging task in practice given the statistical and potentially non-convex nature of the constraint.  Further complicating matters is the fact that by assumption we have access to the data distribution~$\calD$ only through samples~$(\bv x, y) \sim \calD$, which means that in practice we cannot evaluate either of the expectations in~\eqref{P:main}. 

To overcome these obstacles, given a dataset $\{(\mathbf x_n, y_n)\}_{n=1}^N$ sampled i.i.d.\ from $\calD$, our approach is to use duality to approximate~\eqref{P:main} by the following empirical, unconstrained saddle point problem
%
\begin{prob}[$\widehat{\textup{DI}}$]\label{P:empirical_dual}
	\hat{D}^\star = \max_{\nu \geq 0}\ \min_{\btheta \in \Theta}\ \hat{L}(\btheta,\nu)
\end{prob}
%
where the empirical Lagrangian $\hat{L}(\btheta, \nu)$ is defined in the following way:
%
\begin{equation}\label{E:lagrangian}
	\hat{L}(\btheta,\nu) := \frac{1}{N} \sum_{n = 1}^n \left[
	   	\max_{\dinD}\ \ell\big( f_{\btheta}(\bv x_n + \bdelta), y_n \big)
			+ \nu \left[ \ell\big( f_{\btheta}(\bv x_n), y_n \big) - \rho \right]
	\right]
		\text{.}
\end{equation}
%
Thus, in this section, our goal will be to show that solutions of~\eqref{P:empirical_dual} are~(probably approximately) near-optimal \emph{and} near-feasible for~\eqref{P:main}. As one would expect, this is only possible if the objective and constraint of~\eqref{P:main} are learnable individually. As we discussed in Section~\ref{S:problem}, this is known to hold in a variety of scenarios~(e.g., when the Rademacher complexity or VC-dimension are bounded), although obtaining more general results remains an area of active research~\cite{awasthi2020adversarial, yin2019rademacher, cullina2018pac, montasser2020efficiently, montasser2019vc}. To this end, we next formally describe the learning theoretic assumptions we require on the objective and constraint.

\subsection{Learning theoretic assumptions for \texorpdfstring{\eqref{P:main}}{(P-CON)}}

To begin, we assume that the parameterization space $\Theta$ is sufficiently rich, in the sense that a convex combination of any two classifiers $f_{\btheta_1}$ and $f_{\btheta_2}$ can be well-approximated by another classifier $f_{\btheta}$ up to a small, fixed confidence level $\alpha>0$. This is explicitly stated in the following assumption:
%
\begin{assumption}\label{A:parametrization}
The parametrization~$f_{\btheta}$ is rich enough so that for each~$\btheta_1, \btheta_2 \in \Theta$ and~$\beta \in [0,1]$, there exists~$\btheta \in \Theta$ such that
%
\begin{equation}\label{E:approximation_quality}
	\sup_{\bv x \in \calX}\ \abs{\beta f_{\btheta_1}(\bx) + (1-\beta) f_{\btheta_2}(\bx)
		- f_{\btheta}(\bx)} \leq \alpha
		\text{.}
\end{equation}
%
\end{assumption}

\noindent Next, we assume that there exists a parameter $\btheta'\in\Theta$ for which the constraint in~\eqref{P:main} is stictly feasible with margin $\rho - M\alpha$, where $\alpha$ is the constant defined in Assumption~\ref{E:approximation_quality} and $M$ is the Lipschitz constant of $\ell$ with respect to its first argument.  


\begin{assumption}\label{A:slater}
There exists~$\btheta^\prime \in \Theta$ such that~$\E_{\calD} \left[ \ell\big(f_{\btheta^\prime}(\bv x), y\big) \right] < \rho - M\alpha$.
\end{assumption}

\noindent Finally, we make an assumption regarding the concentration of the expectations in the objective and constraint of~\eqref{P:main} around their empirical counterparts.

\begin{assumption}\label{A:empirical}
	There exists~$\zeta_R(N), \zeta_N(N) \geq 0$ monotonically decreasing with~$N$ such that
	%
	\begin{subequations}\label{E:emp_approximation}
	\begin{align}
		\abs{\E_{(\bx,y) \sim \calD} \!\big[ \max_{\dinD}\ \ell\big( f_{\btheta}(\xplusd), y \big) \big]
			- \frac{1}{N} \sum_{n = 1}^{N} \max_{\dinD}\ \ell\big( f_{\btheta}(\bx_n +\bdelta), y_n \big)} &\leq \zeta_R(N)
			\text{ w.p. } 1-\delta
			\label{E:emp_approximation_robust}
		\\
		\abs{\E_{(\bx,y) \sim \calD} \!\big[ \ell(f_{\btheta}(\bv x), y) \big]
			- \frac{1}{N} \sum_{n = 1}^{N} \ell(f_{\btheta}(\bv x_n), y_n)} &\leq \zeta_N(N)
			\text{ w.p. } 1-\delta
			\label{E:emp_approximation_nominal}
	\end{align}
	\end{subequations}
	%
	for all~$\btheta \in \Theta$.
\end{assumption}

\noindent With regard to this final assumption, one natural question to ask is whether the bounds in~\eqref{E:emp_approximation_robust} and~\eqref{E:emp_approximation_nominal} will hold in practice.  To this end, we note that there is overwhelming evidence that the non-adversarial uniform convergence property~\eqref{E:emp_approximation_nominal} holds (see, e.g.,~\cite{bartlett2017spectrally}).  And although these classical learning theoretic results do not imply that the robust uniform convergence property of~\eqref{E:emp_approximation_robust} will hold, there is a growing body of evidence which suggests that this property does in fact hold in practice, and in particular that it holds for the function class of deep neural networks.  Indeed, the results in~\cite{yin2019rademacher,khim2018adversarial,tu2019theoretical} all characterize the sample complexity of the robust learning problem under mild conditions and provide bounds for the specific case in which $\Theta$ is the space of neural networks parameters.


\subsection{Near-optimality and near-feasibility of \texorpdfstring{\eqref{P:empirical_dual}}{(DI)}}

Under these assumptions, we can explicitly bound the empirical duality gap (with high probability) and characterize the feasibility of the empircal dual optimal solution for~\eqref{P:main}.
%
\begin{proposition}[The empirical dual of~\eqref{P:main}]\label{T:dual}
Let~$\ell(\cdot,y)$ be a convex function for all~$y \in \calY$. Under Assumptions~\ref{A:parametrization}--\ref{A:empirical}, it holds with probability~$1-5\delta$ that

\begin{enumerate}
	\item $\abs{P^\star - \hat{D}^\star} \leq M \alpha + (1 + \bar{\nu}) \max(\zeta_R(N), \zeta_N(N))$; and

	\item there exists~$\btheta^\dagger \in \argmin_{\btheta \in \Theta} \hat{L}(\btheta, \hat{\nu}^\star)$ such that~$\E_{(\bv x,y) \sim \calD} \left[ \ell\big(f_{\btheta^\dagger}(\bv x), y\big) \right] \leq \rho + \zeta_N(N)$.
\end{enumerate}
%
\noindent Here, $\hat{\nu}^\star$ denotes a solution of~\eqref{P:empirical_dual}, $\nu^\star$ denotes an optimal dual variable of~\eqref{P:main} solved over~$\bar\calH = \conv(\calH)$ instead of~$\calH$, and~$\bar{\nu} = \max(\hat{\nu}^\star,\nu^\star)$. Additionally, for any interpolating classifier~$\btheta^\prime$, i.e.\ such that $\E_{(\bv x,y) \sim \calD} \left[ \ell\big(f_{\btheta^\prime}(\bv x), y\big) \right] = 0$, it holds that
%
\begin{equation}\label{E:nu_bound}
	\nu^\star \leq \rho^{-1} \E_{(\bv x, y) \sim \calD} \Big[
    	\max_{\dinD}\ \ell\big( f_{\btheta^\prime}(\xplusd), y \big)
    \Big]
    	\text{.}
\end{equation}
%
\end{proposition}

\begin{proof}
	The proof is provided in Appendix~D.
\end{proof}

\noindent At a high level, Proposition~\ref{T:dual} tells us that it is possible to learn robust models with high clean accuracy using the empirical dual problem in~\eqref{P:empirical_dual} at essentially no cost in the sample complexity.  More specifically,  this means that seeking a robust classifier with a given nominal performance is~(probably approximately) equivalent to seeking a classifier that minimizes a combination of the nominal and adversarial empirical loss.  


The majority of past approaches for solving~\eqref{P:main} cannot be endowed with similar guarantees in the spirit of Proposition~\ref{T:dual}.  Indeed, while~\eqref{E:lagrangian} resembles a penalty-based formulation such as TRADES\footnote{Recall that the objective in TRADES seeks an invariant classifier, i.e.\ a classifier for which~$f_{\btheta}(\xplusd)$ and~$f_{\btheta}(\bv x)$ are similar, rather than one with small adversarial loss. This problem can also be accounted for in~\eqref{P:main} by replacing the loss in the objective by a measure of average causal effect~(ACE).}, ALP, CLP, and MART (to name only a few)~\cite{zhang2019theoretically,kannan2018adversarial,wang2019improving}, notice that~$\nu$ is an \emph{optimization variable} in~\eqref{P:empirical_dual} rather than a fixed hyperparameter.  Concretely, the magnitude of this dual variable $\nu$ quantifies the extent to which the sample complexity depends on how hard it is to learn an adversarially robust model while maintaining strong nominal performance.  Though seemingly innocuous, this caveat is the difference between guaranteeing generalization only on the aggregated loss~\eqref{E:lagrangian} and guaranteeing generalization for the objective value and feasibility in the constraint. 



While some pieces of the proof of Proposition~\ref{E:nu_bound} follow from standard learning theoretic techniques, several aspects of the proof are highly nontrivial.  Firstly,~\eqref{P:main} is a nonconvex problem for modern function classes, and therefore it is not immediate that strong duality holds with respect to the dual problem.  Furthermore, note that the guarantees in Proposition~\ref{T:dual} hold  simultaneously for clean and adversarial accuracy, in contrast to regularized approaches. From a learning theoretic perspective, dual learning therefore does as well as currently used (unconstrained) ERM approaches, but with the added advantage that it provides guarantees on the clean and adversarial accuracy separately rather than on a combination of these objective.  To prove that these properties hold simultaneously, we argue that the dual problem is sufficiently regular (see Appendix~\ref{app:prelims-3.6}), which sets the stage for the proof of near-optimality and near-feasibility in Proposition~\ref{T:dual}.
